Conversational Product Search Based on Negative Feedback

Intelligent assistants change the way people interact with computers and make it possible for people to search for products through conversations when they have purchase needs. During the interactions, the system could ask questions on certain aspects of the ideal products to clarify the users' needs. For example, previous work proposed to ask users the exact characteristics of their ideal items before showing results. However, users may not have clear ideas about what an ideal item looks like, especially when they have not seen any item. So it is more feasible to facilitate the conversational search by showing example items and asking for feedback instead. In addition, when the users provide negative feedback for the presented items, it is easier to collect their detailed feedback on certain properties (aspect-value pairs) of the non-relevant items. By breaking down the item-level negative feedback to fine-grained feedback on aspect-value pairs, more information is available to help clarify users' intents. So in this paper, we propose a conversational paradigm for product search driven by non-relevant items, based on which fine-grained feedback is collected and utilized to show better results in the next iteration. We then propose an aspect-value likelihood model to incorporate both positive and negative feedback on fine-grained aspect-value pairs of the non-relevant items. Experimental results show that our model is significantly better than state-of-the-art product search baselines without using feedback and those baselines using item-level negative feedback.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> problem.tex <==
%!TEX root=ProductSearch.tex
\section{Problem Formalization}
%\label{subsec:problem_form}
\begin{comment}
*Problem Formulation
The paradigm of converstional product search based on negative feedback. 
A diagram shows the flow of the search process. 
Illustration of the process. 

Show an example?

Notation and Statement.
Formally state the problem. 
consider a notation table. 
iterative search. 

show how many results each time. 
We consider 1 in this paper. 

Aspect Value Selection. (System ask which aspect values)
Rank the rest items with the preference on the given aspect value
mention that we use semi-synthetic data to do this
\end{comment}

%\subsection{Conversation Search Paradigm Based on Negative Feedback}
%TODO: Illustrate the process
%\subsection{Notation and Statement of the Problem}
%aspect-value pairs are extracted from user review. 
%\label{subsec:notation_prob}
A conversation is initiated with a query $Q_0$ issued by a user $u$. In the $k$-th iteration, a batch of results $D_k$ are retrieved and shown to the user. When $D_k$ does not satisfy the user need, from all the shown non-relevant results, $D_1 \cup D_2 \cdots \cup D_{k}$, denoted as $D_{1:k}$, the system extracts a set of aspect-value pairs, namely, $AV(D_{1:k})$.
Then the system selects $m$ aspect-value pairs $\{(a_{k,j}, v_{k,j})|1\leq j \leq m\}$ from $AV(D_{1:k})$ and asks $m$ corresponding questions $\{Q(a_{k,j}, v_{k,j})|1\leq j \leq m\}$ to the user about whether she likes the aspect-value pairs of the non-relevant results.
After collecting the user's feedback to $Q(a_{k,j}, v_{k,j})$, denoted as $I(a_{k,j}, v_{k,j})$, in the $k+1$-th iteration, the goal of the system is to show a list of results $D_{k+1}$, which ranks the finally purchased item $i$ of the user $u$ associated with $Q_0$ on the top. 
The sequence of actions in the conversation can be represented with 
\begin{equation*}
\label{eq:conv_seq}
\begin{aligned}
% & u \rightarrow Q_0 \rightarrow \cdots D_k Q(a_{k,j}, v_{k,j})\rightarrow I(a_{k,j}, v_{k,j}) \cdots \\ 
u \rightarrow Q_0; \; & D_1, Q_{1,1}, I_{1,1}, \cdots, Q_{1,m} I_{1,m}; \; \cdots; \\ 
							    &D_k, Q_{k,1}, I _{k,1}, \cdots, Q_{k,m}, I_{k,m} \rightarrow i
\end{aligned}
\end{equation*}
where $Q_{k,j}$ and $I_{k,j}$ denote $Q(a_{k,j}, v_{k,j})$ and $I(a_{k,j}, v_{k,j})$ respectively. $Q_{k,j}$ is a yes-no question and $I_{k,j}$ can be $1$ or $-1$ to indicate that the answer is yes or no to the question. 
%$R_u$ and $R_i$ are the historical reviews associated with $u$ and $i$ respectively, which can be used to represent $u$ and $i$

In this paper, we focus on the scenario where only one result is retrieved during each iteration, namely $|D_k| = 1$. However, the method we propose can cope with general cases with more than one result retrieved in each iteration. 

%TODO: semi-sythetic data

